Analytical Performance Models for NoCs with Multiple Priority Traffic Classes

Networks-on-chip (NoCs) have become the standard for interconnect solutions in industrial designs ranging from client CPUs to many-core chip-multiprocessors. Since NoCs play a vital role in system performance and power consumption, pre-silicon evaluation environments include cycle-accurate NoC simulators. Long simulations increase the execution time of evaluation frameworks, which are already notoriously slow, and prohibit design-space exploration. Existing analytical NoC models, which assume fair arbitration, cannot replace these simulations since industrial NoCs typically employ priority schedulers and multiple priority classes. To address this limitation, we propose a systematic approach to construct priority-aware analytical performance models using micro-architecture specifications and input traffic. Our approach consists of developing two novel transformations of queuing system and designing an algorithm which iteratively uses these two transformations to estimate end-to-end latency. Our approach decomposes the given NoC into individual queues with modified service time to enable accurate and scalable latency computations. Specifically, we introduce novel transformations along with an algorithm that iteratively applies these transformations to decompose the queuing system. Experimental evaluations using real architectures and applications show high accuracy of 97% and up to 2.5x speedup in full-system simulation.

==> files/4by4.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}{0.43\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{figures/user_5000_date_11_etarget_8.eps}
		\caption{Energy allocation in January without learning the user 
			pattern.}
		\label{fig:typ_1_1}
	\end{minipage}
	\hspace{1cm}
	\begin{minipage}{0.43\textwidth}
		\centering	
		\includegraphics[width=0.85\linewidth]{figures/user_5000_date_77_etarget_8.eps}
		\caption{Energy allocation in July without learning the user 
			pattern.}
		\label{fig:typ_1_2}
	\end{minipage}
	\vspace{4mm}
	\begin{minipage}{0.43\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{figures/per_user_5000_date_11_etarget_8.eps}
		\caption{Energy allocation in January after learning the user 
			pattern.}
		\label{fig:typ_2_1}
	\end{minipage}
	\hspace{1cm}
	\begin{minipage}{0.43\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{figures/per_user_5000_date_77_etarget_8.eps}
		\caption{Energy allocation in July after learning the user 
			pattern.}
		\label{fig:typ_2_2}
	\end{minipage}
	\vspace{-6mm}
\end{figure*}

==> files/assumptions_notations.tex <==


The proposed performance analysis technique consists of two major steps. 
We first 




\begin{table}[H]
	\caption {Symbols of notations}
	\label {tab_symbols_used}
	\begin{tabular}{|l|p{7cm}|}
		\hline
		$\lambda_i$ & Injection rate for tokens of \textit{class i}                             \\ \hline
		$\mu_i$     & Service rate of \textit{class i}                                          \\ \hline
		$R$                         & Residual time                                                    \\ \hline
		$M_i(t)$                   & Total no. of packets of \textit{class i} injected in the system at time t \\ \hline
		$\rho_i$    & Server utilization for tokens of \textit{class i}                         \\ \hline
		$W_i$                      & Waiting time for tokens of \textit{class i}                               \\ \hline
		$T$                         & Service time                                                     \\ \hline
		TS                        & Structural transformation                                        \\ \hline
		TR                        & Service rate transformation                                      \\ \hline
	\end{tabular}
\end{table}

In table \ref {tab_symbols_used}, we have summarized all the symbols used throughout the paper and their meaning. In this work, we have assumed that each queue is non-preemptive in nature and follows FCFS policy. Also, each transaction happens in each clock ticks i.e. the queuing system operates based on discrete timing. As in realistic NoC designs tokens are served in fixed number of cycles, we are taking deterministic service time for subsequent calculations. Though in industrial design, queue sizes are limited to 16 or 32 we are assuming infinite queues for the proposed technique. But we also observe that usually queue length does not grow beyond around 30 tokens closed to saturation.

In this work, we are dealing with priority based queuing network. We are formally modeling priority based network through xMAS notations as described in \cite {chatterjee2012xmas}. In xMAS notation, there are small set of primitives which are sufficient to describe a queuing system. Main advantage of xMAS is modeling is quick since it is high level. Figure \ref {fig_xmas_primitives} shows the primitives used throughout the paper and figure \ref {fig_example_xmas} is an example of a priority based queuing system modeled through xMAS. In this system tokens of \textit{class x} have higher priority than tokens of \textit{class y} i.e. tokens of \textit{class y} will not be served till all the tokens of \textit{class x} in the queue are served.

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
	\centering
	\resizebox{0.50\textwidth}{!}{\includegraphics[width=0.5\textwidth]{figures/xmas_primitives.eps}}
	\caption{xMAS primitives used}
	\label{fig_xmas_primitives}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
	\centering
	\resizebox{0.50\textwidth}{!}{\includegraphics[width=0.5\textwidth]{figures/example_xmas.eps}}
	\caption{Usage of XMAS modeling}
	\label{fig_example_xmas}
\end{subfigure}
\caption {xMAS modeling and its use}
\end{figure}
